Stochastic Wavevector Model for Rapidly-Distorted Compressible Turbulence

A stochastic wavevector approach is formulated to accurately represent compressible turbulence subject to rapid deformations. This approach is inspired by the incompressible particle representation model of Kassinos (1995) and preserves the exact nature of compressible Rapid Distortion Theory (RDT). The adoption of a stochastic - rather than the Fourier - perspective simplifies the transformation of statistics to physical space and serves as a starting point for the development of practical turbulence models. We assume small density fluctuations and isentropic flow to obtain a transport equation for the pressure fluctuation. This results in five fewer transport equations compared to the compressible RDT model of Yu and Girimaji (2007). The final formulation is closed in spectral space and only requires numerical approximation for the transformation integrals. The use of Monte Carlo for unit wavevector integration motivates the representation of the moments as stochastic variables. Consistency between the Fourier and stochastic representation is demonstrated by showing equivalency between the evolution equations for the velocity spectrum tensor in both representations. Sample clustering with respect to orientation allows for different techniques to be used for the wavevector magnitude integration. The performance of the stochastic model is evaluated for axially-compressed turbulence, serving as a simplified model for shock-turbulence interaction, and is compared to LIA and DNS. Pure and compressed sheared turbulence at different distortion Mach numbers are also computed and compared to RDT/DNS data. Finally, two additional deformations are applied and compared to solenoidal and pressure-released limits to demonstrate the modeling capability for generic rapid deformations.

==> RevisionResponses.tex <==
Referee: 1

Comments to the Author
This work develops a stochastic model for compressible turbulence that is valid in the rapid distortion limit. The authors discuss the equivalency of stochastic sample space to the Fourier space and discuss the advantages a stochastic approach offers, especially for numerical integration. They also demonstrate that the model is well-behaved in homogeneous turbulence: axial compression, shear, and combined compression and shear.

RESPONSE: The authors appreciate the thoughtful reviews. A point-by-point response is below


While the novelty of the methodology is clear, the application of the model in inhomogeneous flows does not seem possible in the first glance (for example: equations 3.14 – 3.19 can’t remain in pure spectral space in inhomogeneous flows). It would be beneficial for the reader if the authors expound on how this model is readily applicable for inhomogeneous flows.  

RESPONSE: Thank you for bringing this up. Application to inhomogeneous flows can be done in several ways and will be explored in future work. A paragraph on the extension of the current method to inhomogeneous flows (and nonlinearity) is given in lines 874-891. While the referee is correct that the exact equations presented can (likely) not be used directly in inhomogeneous formulation, a similar set of equations can be derived by using a non-periodic basis such as Chebyshev polynomials instead of a Fourier basis. This of course, may change the equations and is actively being explored. Another way that the equations can be applied to inhomogeneous flows is using a quasi-homogeneous approach similar to Durbin's elliptic-relaxation technique. The last paragraph goes over this in detail.

Introduction:
- what does q stand for?

RESPONSE: $q^2$ is twice the TKE. added definition to line 28

- Line55: ‘RDT is valid when the timescale of turbulent distortion is shorter than time scale of large eddies’. But if you start from the RDT limit S τ>1, then τ>1/S implying that the turbulence time scale is larger. 

RESPONSE: added condition that S tends towards infinity in rapid distortion limit, implying that the turbulent time scale tau is tends toward zero. Lines 33

- Line94: ‘more particles compared’ missing to?
RESPONSE: fixed


Sections 2, 3 and 4 are not very organized. Symbols for certain variables are not carefully chosen (1 symbol for 2 variables, 1 variable has multiple symbols, etc). Overall, this section could also use a bit more restructuring as the reader has to work hard to understand what is unique to the authors’ model and what is already present in the literature (specially in section 4). Some specific comments in this section are listed below:

- Line 149: missing averaging operator over ρ?
- Equation 3.3: missing averaging operator over p?
- Line 174 and beyond:  i is used to denote subscript and $\sqrt(-1)$. Imaginary number is typically denoted by \mathrm{i} as it is an immutable constant.
- k is used for the wavenumber and as a subscript. Would be good if $\kappa$ is used for wavenumber
- In introduction the turbulence time scale was denoted by$ \tau$, whereas in section 3, it is denoted by $\tau_t$
- The upper and lower limits of the integration in equations 3.20 3.21, 3.22 and 3.23 are the same
- The location of subscripts for u in Rij also change (line 186 vs equation 3.9)
RESPONSE: Thank you. We fixed these typos and duplicate variables

- The sample number in line 336 appear as a subscript whereas the particle number in equation 5.1 appears as a superscript. Is there a reason for this choice?
RESPONSE: Did not want to confuse with superscripts as powers, but since sample is denoted by superscript in rest of the paper, this has been changed.

- Line 307: ‘makes it difficult’ missing to?
- The abbreviation PDF is used without introducing it
RESPONSE: fixed minor issues

Section 5:
- Several symbols appear in the Algorithm, especially in Inputs that were not defined before
- There is a lot of white space in Figs. 3 and 5 and could be zoomed in a bit more to see the details. Overall, the quality of all the plots could be improved (thicker linewidths, bigger fonts)


Referee:2

The authors derive and develop a stochastic particle-based method for computing the development of
statistics for compressible homogeneous turbulence using rapid distortion theory (RDT). The authors’
approach to solving the RDT problem is an extension of the method of Kassinos for incompressible flow.
The authors give a good explanation of their method, although some details need to be clarified, as
stated in the list of issues to be addressed below. For several cases with mean flow distortion the authors present computations of various relevant turbulent statistics and make comparisons with
previously published results from direct numerical simulations (DNS) and analytical RDT results in the pressure-released limit and for purely solenoidal turbulence. The authors demonstrate and explain the limitations of their own computations and they discuss limitations of previously DNS and RDT results. Also included are results for two cases where there are no corresponding DNS results.
The authors’ motivation for this work is to aid in the future development of turbulence models for compressible flow, although no direct link is given to the development of turbulence models.
Overall, the paper is interesting and well written. I suggest the paper be accepted for publication once the specific issues listed below are addressed. (The line numbers listed below refer to the editorial line numbers in the margin of the PDF document sent to the reviewers.)\

RESPONSE: The authors appreciate the thoughtful reviews. A point-by-point response is below

1. Line 35: The authors say, “... the turbulence ... behaves more like an elastic solid.” Please provide a reference where that connection is made in more detail.
RESPONSE: added paper by Crow and Taylor that details this behavior in detail. Line 36


2. Line 129: Remove the word “gradient,” since compressible homogeneous turbulence cannot have a mean density or pressure gradient.

RESPONSE: I believe that there can be mean density and pressure gradients in compressible homogeneous turbulence with the requirement that they only vary in time and not space. See the Ph.D. thesis by Blaisdell as cited in the paper for why this is so.


3. Line 170: Please clarify whether equation (3.4), the Poisson  equation for the fluctuating pressure for a solenoidal velocity field, is used in the author’s RDT analysis.

RESPONSE: Clarified that it is used to find solenoidal components only. It is not used in the derivation of the full compressible formulation. Lines 183-184

4. Line 170: There is a “2” missing in the Laplacian operator on the LHS of equation (3.4).
RESPONSE: Fixed

5. Line 170: What is the meaning of the asterisk (*) in the last term on the RHS of equation (3.4).
RESPONSE: this was a typo

6. Line 249: Equation (3.21) makes improper use of index notation, since the index “i” is used three times within the integrand. Instead, a different pair of indices should be used on the velocity
spectrum tensor: Φmmmm .
RESPONSE: this was a typo and is corrected

7. Line 263: The authors say the flow variables are treated as “stationary” random fields. This seems confusing because the turbulence statistics change in time, i.e., they are not stationary.
RESPONSE: UNSURE


8. Lines 297-298: The authors say, “Kassinos (1995) also initialized the ... by a factor of 4π.” Is “initialized” the correct word here? Do the authors mean “scaled” or “normalized”?
RESPONSE: We meant that Kassinos scaled the tensor by 4π in the intialization rather than at each timestep. I have re-worded the sentence. Line 354

9. Line 397: The authors say the joint PDF is “derived using traditional methods ...” Please provide a reference for the sake of readers are not familiar with PDF methods.
RESPONSE: cited the book by Heinz. Line 452

10. Line 511: It is unclear how the initial dilatational velocity spectrum is determined. The authors specify the ratio of the solenoidal and dilatation velocity variances, qqss
2 qqdd 2 ⁄ , as a parameter, and they give possible forms of the velocity spectrum EE(kk) in equations (5.2) and (5.4); however, they do not say whether the initial dilatational velocity spectrum is proportional to the solenoidal spectrum (i.e.,
just scaled in magnitude) or something else is used
RESPONSE: added condition that $E_s/E_d=q_s^2/q_d^2$ so that the velocity spectra are proportional to each other by the same amount as the TKE. Line 569

11. Line 519: Why are different values of the ratio of specific heats chosen for some of the cases?
RESPONSE: this was done to compare against DNS data from different papers. The axial compression DNS data came from a separate paper that used a different ratio from the rest.

12. Line 520: Change “constant mean temperature of TT� = 300” to “constant initial mean temperature of TT� = 300”. (Even though this section describes the methods used for initialization, it still would be helpful to make clear that the mean temperature is not assumed constant throughout the
simulation.)
RESPONSE: added clarification line 580

13. After Line 520: It would be helpful it the authors said how the initial density and temperature fluctuations are determined. Is the isentropic relation used to relate ρρ′ and TT′ to pp′, or is something else done?
RESPONSE: Since density and temperature fluctuations do not appear in the equations, they are not required but can be found using the isentropic reations. Added this to paper lines 580-584

14. Page 15, Algorithm 1: I believe the line with “for t = 1 : nk do” should be “for k = 1 : nk do”.
RESPONSE: correct, this was a typo

15. Line 537: What do the authors mean by “the dilatational mode is balanced by the pressure gradient”?
RESPONSE: It means that the pressure and dilatational modes exchange energy are equivalent and thus the dilatational modes are not required to close the equations. Added citation, line 596-598


16. Lines 550-551: Is the discretization of the wavenumber magnitude uniformly spaced? If not, how is the discretization done?
RESPONSE: it is logarithmically spaced. I have added this detail to the paper line 552

17. Line 594: Remove the word “are” at the end of the line.

18. Line 612: The standard definition of the Reynolds stress anisotropy tensor is
bbiiii = RRiiii − 1
3qq2δδiiii
qq2 .
While Mahesh did compute and plot RRiiii qq2 ⁄ , this quantity was not called bbiiii .
RESPONSE: The Plot axis for Rij/q2 corrected on the axial compression cases and fixed typo

19. Line 791: Why do equations (A 6)-(A 10) not include Φiiii
dd ?
RESPONSE: the ds cross-correlational does not appear when only considering the evolution for the symmetric solenoidal and dilatational velocity spectrum tensors.

20. Lines 811-857: There are several formatting issues that need to be fixed in the Reference list.
RESPONSE: formatting issues fixed

Referee: 3

The study addressed in the manuscript is interesting and deserves publication to the JFM. I
have comments, mainly on the request for a larger review of literature, as follows.
One of the first stochastic wavevector model was proposed by J.C.H. Fung (from his thesis,
1990?) and coworkers , and was coined Kinematic Simulation by Julian Hunt. The Eulerian velocity field is given by a very high number of 3D Fourier components, in which the orientation of the wave vector is chosen randomly. In the seminal approaches, the turbulence was considered isotropic, without effect of mean gradients and/or body forces. Furthermore, the linear dynamics from RDT was incorporated in such anisotropic kinematic simulation, in Cambon et al. (2004) and in Favier et al. (2010), namely (see at the end.) 

Here, the authors mention the method called PRM (Particle Representation Model, from Kassinos 1995, and Kassinos & Reynolds 1996.) In the original approach, Kassinos, Reynolds and coworkers even did not mention the analogy of their PRM model with a Fourier representation: Looking at their equations, it appears that a ‘gradient vector’ a (or k∗ in Fig. 1?) is the surrogate of the orientation of the wavevector, which plays an essential role for taking
into account the pressure fluctuation in incompressible RDT. Note that much more details can be found in the Ph. D report by Stavros Kassinos, but the equivalency with spectral representation is only discussed at length in the book by Sagaut and Cambon (see at the
end).
In compressible turbulence, the wavevector information for inviscid RDT is not restricted to the orientation of the wavevector but calls into play its modulus as well. This additional
complexity is due to the ak parameter, or dispersion frequency of acoustic waves, in linearized spectral equations. Is it possible to identify that term in Eqs. (3.14-3.16)? In this weakly
compressible case , the study in the present ms. shares most of equations and formalism with the articles by Cambon et al. (1993) and Simone et al. (1997), namely, so that its originality
lies in the randomization of the wave vector and in computation of integrals in Fourier space using Monte-Carlo techniques.

RESPONSE: the additional citations have been added to the paper, as well as a few points on the dispersion factor and where it appears in the equations. In the thesis by Kassinos, the equivalency between the stochastic/spectral approaches is demonstrated but not as in much detail as in vanSlootens work. Have also added the Sagaut and Cambon book .

I have more incidental comments as follows:
-) p. 2. ‘Rather than using this decomposition, ... in this reference frame’. The transformation for deforming coordinates is applied as well in all the references mentioned by the authors, that use, in addition, the Craya-Herring local frame of reference. In such a frame, the dilatational part of the velocity field is aligned with the wavevector, whereas two orthogonal solenoidal (divergence free in Fourier space) components lies in the plane normal to the wavevector. This is completely consistent with fig. 1 and the last sentence of p. 9, but more explicit. In addition, the way of initializing random data for isotropic turbulence in Rogallo (1981) can easily be interpreted using the Craya-Herring frame, in spite of different terminology.

RESPONSE: unsure how to respond to this? any changes required?

Section 5, applications. Comparisons are made with DNS of Cambon et al. (1993) and Simone et al. (1997), but RDT is used as well in these studies, using random initialization and integration of spectra. Could the authors discuss a bit more differences and analogies with their own CPRM model?

RESPONSE: Added a paragraph on comparison between the CPRM and RDT of those two papers. In summary, the largest differences is a different set of equations to solve due to the use of Helmholtz decomposition and deforming+Craya-Herring coordinates in Cambon et al. and Jacquin at al. papers versus just the deforming coordinates of the full field in CPRM, and different methods of integration (spectral versus stochastic in the CPRM case). Same set of assumptions and governing equations are used for both and thus why we expect the results to match well.

In short, I recommend publication after a substantial revision, as suggested by my comments Additional references suggested
Favier, B., Godeferd, F.S., Cambon, C.: On space and time correlations of isotropic and
rotating turbulence. Phys. Fluids 22, 015101 (2010)
Cambon, C., Godeferd, F.S., Nicolleau, F., Vassilicos, J.C.: Turbulent diffusion in rapidly
rotating flows with and without stable stratification. J. Fluid Mech. 499, 231255 (2004)
Sagaut, P., and Cambon, C. 2018. Homogeneous turbulence dynamics (monograph), Springer.


Referee: 4

Comments to the Author
The authors derive the compressible RDT (Rapid Distortion Theory) equations by linearizing the Navier-Stokes equations about the Reynolds-averaged state variables and invoking isentropic flow simplifications. The isentropic assumption simplifies the governing equations to some extent compared to the ideal gas equation of state used in prior studies. To solve the RDT equations, the authors employ the particle representation method. In contrast to previous approaches, they generate the wave-vector initial conditions by randomly sampling within a specified function space. It appears that a closed set of spectral second-moment equations is solved, rather than the velocity perturbation equations. This definitely is an interesting novelty. The resulting compressible RDT computational results from axial compression, pure shear, and sheared compression cases, are presented and compared to some data in the literature. While there is adequate agreement in some of the statistical comparisons, marked differences are observed in other cases.

Overall, the paper introduces an interesting variation of current compressible RDT computations. The manuscript would benefit from significant revisions to address the issues outlined below.

1. Fundamental limitations of employing (i) linearization about the Reynolds averaged velocity field for compressible turbulence analysis and (ii) isentropic assumptions should be explicitly discussed. In axisymmetric compression case, the background density increases substantially, and the fluctuating field is also likely to exhibit high density magnitudes. Further, is the degree of simplification afforded by the isentropic assumption substantial enough to offset the limitations? Previous works have shown that the ideal gas RDT equations permit elegant analysis in many cases.
RESPONSE: Added a section on limitations starting line 280. (i) Explicitly discussed limitations of linearization and how we can interpret it as a first-step towards a turbulence model that behaves correctly in the limit of large distortions. (ii) The isentropic relation relating to the change in density fluctuation is further explained in that it is weakly enforced i.e. the terms in the velocity fluctuation  evolution equation containing the density fluctuation are small in comparison to the other terms, but the density fluctuation is not zero as evidenced by the need to evolve the pressure fluctuation with respect to density fluctuation. We also discuss in detail how much this simplification reduces the number of equations.

2. The pure shear kinetic energy evolution comparison presented in figures 7a (CPRM-RDT), 7b (DNS) and figure 8 indicate serious disagreement. The authors speculate that there may be errors in the DNS data of Simone et. al (1997). The authors would benefit from comparing their results with the more recent and accurate RDT and DNS results of Lavin et. al (TCFD, 2011), Bertsch et. al (POF, 2012) and Kumar et. al (JFM, 2014). These papers are directly related to the present paper and provide more recent validation data. Indeed, the authors will find much better agreement.
RESPONSE: The agreement with the DNS TKE evolution from Simone et. al (1997) is indeed poor, however the RDT data (the b12 component evolution) from the same paper is an adequate comparison. Our results were not as good as they can be, and have been improved by solving the wavevector modulus evolution equation and varying the modulus (as appearing in equations 4.9-4.11) for each cluster. TKE evolution is replotted as well and additional citations are used to compare

3. The authors should further explain the flow physics of the `cross-over’ point (Fig. 8a) and the intermediate flattening of the kinetic energy evolution (Fig. 7a). A clear physical rationale for these observations has been developed in the above three references. A detailed analysis has been performed to show that flow-thermodynamic interactions lead to the observed behavior.  Addition of a succinct flow-physics discussion on the three-stage velocity-pressure field interaction (along the lines presented in the references) will add significantly to overall completeness of the paper.
RESPONSE: A discussion of the flow physics talking about the crossover point and TKE flattening has been added lines 707-727 and lines 741-756

4. The authors should also consider including pressure statistics and examine the partition of energy between internal and dilatational-kinetic energies. The equipartition of energy between these modes in the intermediate stage (plateau of kinetic energy evolution) should be investigated.
RESPONSE: Equipartition and pressure statistics has been added with figures 10 and 11, along with brief discussion

Minor comments:

1. The nomenclature of `Stochastic Wavevector Model’ is somewhat misleading. The authors have adapted the terminology from Kassinos and Reynolds. However, in most literature, a stochastic model is one in which the solution experiences random perturbations over time. In this case, the randomness is only in the choice of initial conditions and the system evolves deterministically.
RESPONSE: Correct, have added to the paragraph in the introduction to make this distinction explicit lines 51-54

2. The authors should consider editing Section 4 to simplify the explanation of the current model and integrate it with Section 5.2 which provides the model algorithm. Is it necessary to express statistical evolution using integrals in the context of a discrete particle method? Is a simpler explanation possible? In traditional approach, the Parseval theorem is used to infer the statistics in physical space from wavevector ensembles.

3. The authors should also verify the precision of several statements in Section 4. For example,
a. At the beginning of Section 4, it is stated that `In stochastic representation, flow variables are treated as stationary random fields’. Clearly, the velocity perturbations grow unbounded.  
b. Above Equation 4.1, it is stated that in previous methods `Fourier modes must be integrated with respect to all wave-vectors’. The traditional methods solve directly for conditional velocity amplitude of a given wave-vector and use Parseval theorem leading to a simple summation rather than an integration over wavevectors.

RESPONSE: unsure how to add these changes
